Post-Processing of High-Dimensional Data

Scientific computations or measurements may result in huge volumes of data. Often these can be thought of representing a real-valued function on a high-dimensional domain, and can be conceptually arranged in the format of a tensor of high degree in some truncated or lossy compressed format. We look at some common post-processing tasks which are not obvious in the compressed format, as such huge data sets can not be stored in their entirety, and the value of an element is not readily accessible through simple look-up. The tasks we consider are finding the location of maximum or minimum, or minimum and maximum of a function of the data, or finding the indices of all elements in some interval --- i.e. level sets, the number of elements with a value in such a level set, the probability of an element being in a particular level set, and the mean and variance of the total collection. The algorithms to be described are fixed point iterations of particular functions of the tensor, which will then exhibit the desired result. For this, the data is considered as an element of a high degree tensor space, although in an abstract sense, the algorithms are independent of the representation of the data as a tensor. All that we require is that the data can be considered as an element of an associative, commutative algebra with an inner product. Such an algebra is isomorphic to a commutative sub-algebra of the usual matrix algebra, allowing the use of matrix algorithms to accomplish the mentioned tasks. We allow the actual computational representation to be a lossy compression, and we allow the algebra operations to be performed in an approximate fashion, so as to maintain a high compression level. One such example which we address explicitly is the representation of data as a tensor with compression in the form of a low-rank representation.

==> chapters/coefficients.tex <==
% RCSID:       $Id: coefficients.tex,v 1.3 2015/08/08 20:48:25 hgm Exp $
% Author:      
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.3 $",
%%  DATE      = "$Date: 2015/08/08 20:48:25 $",
%%  FILENAME  = "$RCSfile: coefficients.tex,v $"}

\section{Coefficients} \label{S:coeff}
%

  \note{to be written initially by Alexander Litvinenko}


The coefficients  ...

This was to cover the case when we do not have directly a low-rank
representation of the samples $\tnb{w}$, but the samples are generated
by evaluating a \emph{functional representation}
\[ w(\vek{p}) = \sum_{m_1,\dots,m_d}  u_{m_1,\dots,m_d}
  \,  \psi_{m_1,\dots,m_d}(\vek{p}), \]
and we have a low-rank representation of the coefficients $\tnb{u}=(u_{m_1,\dots,m_d})$.


%  $Log: coefficients.tex,v $
%  Revision 1.3  2015/08/08 20:48:25  hgm
%  notes included
%
%  Revision 1.2  2014/08/27 20:23:39  hgm
%  set-up completed
%
%  Revision 1.1  2014/08/27 20:11:15  hgm
%  initial check-in
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../14_tensor_post-proc"
%%% End: 


==> chapters/not_used_truncation.tex <==
% RCSID:       $Id: truncation.tex,v 1.3 2015/08/08 20:52:45 hgm Exp $
% Author:      
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.3 $",
%%  DATE      = "$Date: 2015/08/08 20:52:45 $",
%%  FILENAME  = "$RCSfile: truncation.tex,v $"}

\section{Truncation} \label{S:trunc}
%
\note{Describe how truncation is working for these formats.}
%
In \cite{Kressner17_Trunc} the authors suggeste a new recompression randomized algorithm for Tucker and TT tensor formats.
%
\subsection{Truncation in Tucker tensor format}
%
\subsection{Truncation in Tensor Train format}


%  $Log: truncation.tex,v $
%  Revision 1.3  2015/08/08 20:52:45  hgm
%  notes included
%
%  Revision 1.2  2014/08/27 20:23:31  hgm
%  set-up completed
%
%  Revision 1.1  2014/08/27 20:10:30  hgm
%  initial check-in
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../14_tensor_post-proc"
%%% End: 


==> common/default-commands.tex <==
% RCSID:       $Id$
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% Some default LaTeX commands for every day use

\newcommand{\Index}[1]{\emph{#1}\index{#1}}
\newcommand{\IndexT}[2]{\emph{#1}\index{#2}}
\newcommand{\IndexExt}[2]{\emph{#1#2}\index{#1}}
\newcommand{\IndexSee}[2]{\emph{#1}\index{#1|see{#2}}}
\newcommand{\IndexPerson}[2]{\emph{#1}\index{#2}}
\newcommand{\indexbf}[1]{{\bf #1}}
\newcommand{\indexit}[1]{{\it #1}}

\newcommand{\bv}[1]{\mathbf{#1}}
\newcommand{\namedspace}[1]{\mathcal{#1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\true}{true}
\DeclareMathOperator*{\false}{false}


==> common/easy-defaults.tex <==
% RCSID:       $Id: easy-defaults.tex 32 2007-03-15 16:51:55Z opajonk $
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% Common settings

\tolerance=10000
\emergencystretch=14pt

==> common/pdfsetup.tex <==
% RCSID:       $Id: pdfsetup.tex 36 2007-04-12 15:00:01Z opajonk $
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% Setup PDF-Latex to fill in all relevant metadata into a PDF file
%
% Needs: - you have to declare \theauthor, \thetitle, \thesubject
%           \pdflinkcolor and  \thekeywords before including this file

% The following package defines \ifpdf properly even with MikTeX 2.5
\usepackage{ifpdf}

\ifpdf
  \usepackage[pdftex,
       colorlinks=true,		% use links with color instead of boxes
       bookmarksnumbered,	% bookmarks have numbers in front of topic
       bookmarksopen,		% opens the bookmarks when the PDF is opened
       pdfstartview=FitH,	% opens the PDF with 'fit width' view
       linkcolor=\pdflinkcolor,	% standard red
       citecolor=\pdflinkcolor,	% standard green
       urlcolor=\pdflinkcolor,	% standard cyan
       filecolor=\pdflinkcolor,	% ?
       hyperindex,		% ?
       plainpages=false,	% ?
       breaklinks=true,		% allow links to break across lines!
       pdfpagelabels, %?
       hypertexnames=true,
%        linktocpage=true  % if enabled the link in toc is placed on the number rather than on the text
     ]{hyperref}
     \pdfinfo{
        /Title (\thetitle)
        /Author (\theauthor)
        /Subject (\thesubject)
        /Keywords (\thekeywords)}
     \usepackage[dvipdf]{graphicx}
	 \usepackage[pdftex]{thumbpdf}
\else
  \usepackage[
    colorlinks=true,
    linkcolor=\pdflinkcolor,
    hyperindex,
    plainpages=false
  ]{hyperref}
  \usepackage[dvips]{graphicx}
\fi

\hypersetup{a5paper,
            colorlinks,
            linkcolor=\pdflinkcolor,
            citecolor=\pdflinkcolor,
            urlcolor=\pdflinkcolor,
            pdftitle={\thetitle},
            pdfauthor={\theauthor},
            pdfsubject={\thesubject},
            pdfkeywords={\thekeywords},
            pdfproducer={\theauthor~using \LaTeXe}}


==> config.tex <==
% RCSID:       $Id: config.tex.in 32 2007-03-15 16:51:55Z opajonk $
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% =============================================================================
% Variables to steer output

%pdflinkcolor={blue|black}
% Set to blue to create a PDF for on screen viewing
% or to black for printing
\newcommand{\pdflinkcolor}{blue}



%  $Log$
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "11_tens-rep-calc"
%%% End: 


